RAMP: Hierarchical Reactive Motion Planning for Manipulation Tasks Using Implicit Signed Distance Functions

We introduce Reactive Action and Motion Planner (RAMP), which combines the strengths of sampling-based and reactive approaches for motion planning. In essence, RAMP is a hierarchical approach where a novel variant of a Model Predictive Path Integral (MPPI) controller is used to generate trajectories which are then followed asynchronously by a local vector field controller. We demonstrate, in the context of a table clearing application, that RAMP can rapidly find paths in the robot's configuration space, satisfy task and robot-specific constraints, and provide safety by reacting to static or dynamically moving obstacles. RAMP achieves superior performance through a number of key innovations: we use Signed Distance Function (SDF) representations directly from the robot configuration space, both for collision checking and reactive control. The use of SDFs allows for a smoother definition of collision cost when planning for a trajectory, and is critical in ensuring safety while following trajectories. In addition, we introduce a novel variant of MPPI which, combined with the safety guarantees of the vector field trajectory follower, performs incremental real-time global trajectory planning. Simulation results establish that our method can generate paths that are comparable to traditional and state-of-the-art approaches in terms of total trajectory length while being up to 30 times faster. Real-world experiments demonstrate the safety and effectiveness of our approach in challenging table clearing scenarios. Videos and code are available at: https://samsunglabs.github.io/RAMP-project-page/

==> 3-problem-statement.tex <==
\section{Problem Statement}
\label{sec:problem-statement}

\vtxt{This section reads more like a "motivating application" section than a problem statement section.}

\subsection{Table Clearing Task}
In this work, we consider a robot that needs to autonomously clear a table by picking up objects from clutter, remove any leftover items by dropping them in a trash can, and then load the objects in the dishwasher, without any human interventions. We use the following object classes: plates, bowls, mugs, forks, spoons, and knives. The robot is equipped with a wrist camera for observing objects on the table, and our setup also includes an external camera for observing the whole scene and detecting other obstacles in the environment.

Since the main focus of this paper is on reactive motion planning, we assume the existence of off-the-shelf semantic segmentation \cite{KaimingGkioxari_MaskRCNN_2017} and object pose estimation \cite{He_FFB6D_2021} algorithms, trained on objects that the robot might encounter in the scene. Additionally, we use a grasping module, that proposes feasible grasps based on the detected object class, and a placement module, that proposes feasible leftover disposal and dishwasher placement poses. The robot needs to pick, dispose of leftover items and place objects sequentially, with a pre-defined picking logic.

Within this complicated system, we found that traditional motion planning approaches, such as RRT \cite{LaValle_Planning_2006} or RRT* \cite{KaramanFrazzoli_RRTstar_2010}, are insufficient, since the robot sometimes operates very close to its joint limits where sampling is problematic (e.g., when placing bowls in the dishwasher or when picking up plates from the table) and needs to account for several constraints (e.g., the leftovers need to remain inside the plate before disposal). Typically, in such conditions, these algorithms spend a lot of time planning and, even when they find a solution, a separate optimization module is needed to design a joint-space trajectory that follows the generated path without violating any kinematic or dynamic constraints. Additionally, there is no way to adjust online to changed obstacles in the scene, as the robot navigates to a given target.

\subsection{Motion Planning Task}
During an execution of the table clearing task, the motion planner is needed in order to navigate to a feasible end-effector grasping, leftover disposal or dishwasher placement pose. We transform such a pose target to the robot's configuration space $\mathcal{C}$ using inverse kinematics (e.g., with IKFast \cite{Diankov_IKFast_2010}), to get an array of target joint angles, $\mathbf{q}_{\text{goal}} \in \mathcal{C}$.

For obstacle avoidance purposes, we consider the whole scene as a large point cloud. This point cloud is constructed by concatenating points sampled from meshes of known objects in the scene (e.g., the table or the dishwasher tray), with the point clouds of objects on the table (observed by the wrist camera) and external obstacles (observed by the external camera). Finally, assuming the presence of a low-level joint torque controller that can achieve commanded joint velocities $\mathbf{u} \in T\mathcal{C}$, we consider a first-order, fully-actuated abstraction of the robot for motion planning purposes, as $\dot{\mathbf{q}} = \mathbf{u}$.

With this description, our task at each control timestep, given the current scene point cloud and robot configuration $\mathbf{q} \in \mathcal{C}$, is to generate a velocity command $\mathbf{u}$ that drives the robot to the target $\mathbf{q}_{\text{goal}}$, while avoiding obstacles in the environment and respecting any configuration constraints (such as maintaining a desired end-effector pose), as well as the joint position and velocity limits of the robot.

==> discussion.tex <==
\vtxt{General Discussion and Comments}

\subsection{High level motivation}
For company-level planning I think we need to motivate the problem more strongly from an application point of view. Perhaps we can use the benchmark for this purpose: give examples of challenging instances where finding a feasible path is very challenging due to not just workspace but also configuration space narrow passages. Then, we can say something about the state of the art methods. It takes them a long time but they also recompute from scratch 

\subsection{A research idea}
As humans we don't necessarily avoid collisions during manipulation planning --eg when we reach into the fridge. This is something that we can play with since it plays nicely with the challenges of SDF. Rather than learning very fine details, we can go ahead and plan with coarse representations and let feedback and online planning help later on. This also opens up the possibility to use novel distance functions. For example instead of $\min{x,y}$ we can use a weighted average of the distances of the control points. Collisions with the gripper are not so bad perhaps (because we can adjust the motion more easily) but a collision with an elbow is worse.
